Milestones over Outcome: Unlocking Geometric Reasoning with Sub-Goal Verifiable Reward

Multimodal Large Language Models (MLLMs) struggle with complex geometric reasoning, largely because "black box" outcome-based supervision fails to distinguish between lucky guesses and rigorous deduction. To address this, we introduce a paradigm shift towards subgoal-level evaluation and learning. We first construct GeoGoal, a benchmark synthesized via a rigorous formal verification data engine, which converts abstract proofs into verifiable numeric subgoals. This structure reveals a critical divergence between reasoning quality and outcome accuracy. Leveraging this, we propose the Sub-Goal Verifiable Reward (SGVR) framework, which replaces sparse signals with dense rewards based on the Skeleton Rate. Experiments demonstrate that SGVR not only enhances geometric performance (+9.7%) but also exhibits strong generalization, transferring gains to general math (+8.0%) and other general reasoning tasks (+2.8%), demonstrating broad applicability across diverse domains.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/00_abstract.tex <==
\begin{abstract}
% Multimodal Large Language Models (MLLMs) currently struggle with complex geometric reasoning, largely because training relies on sparse, outcome-based feedback. This paradigm fails to penalize flawed reasoning that coincidentally yields correct answers or reward sound logic that results in minor calculation errors. To address this, we propose shifting from outcome-only to subgoal-level supervision. We introduce a new geometric reasoning benchmark where each problem is paired with a formally verified, step-wise proof skeleton. By mapping abstract geometric predicates to verifiable numerical sub-goals, we generate dense, trustworthy subgoal-level supervision. Leveraging this data, we propose the \textbf{S}ub\textbf{G}oal-Level \textbf{V}erifiable \textbf{R}eward (SGVR) framework. SGVR utilizes reinforcement learning with a novel dense reward signal---the \textit{Skeleton Rate}---to optimize the proportion of correctly derived intermediate steps. Experiments demonstrate that SGVR significantly improves both final-answer accuracy and reasoning quality across diverse geometry, math, and logic benchmarks, consistently outperforming strong baselines. Our work offers a verifiable benchmark and a robust training framework, establishing subgoal-level supervision as a key to unlocking MLLM reasoning capabilities.

Multimodal Large Language Models (MLLMs) struggle with complex geometric reasoning, largely because "black box" outcome-based supervision fails to distinguish between lucky guesses and rigorous deduction. To address this, we introduce a paradigm shift towards subgoal-level evaluation and learning. We first construct \textit{GeoGoal}, a benchmark synthesized via a rigorous formal verification data engine, which converts abstract proofs into verifiable numeric subgoals. This structure reveals a critical divergence between reasoning quality and outcome accuracy. Leveraging this, we propose the \textbf{S}ub-\textbf{G}oal \textbf{V}erifiable \textbf{R}eward (SGVR) framework, which replaces sparse signals with dense rewards based on the \textit{Skeleton Rate}. Experiments demonstrate that SGVR not only enhances geometric performance (\textbf{+8.1\%}) but also exhibits strong generalization, transferring gains to general math (\textbf{+8.0\%}) and other general reasoning tasks (\textbf{+2.8\%}), demonstrating broad applicability across diverse domains.
\end{abstract}




==> sections/01_intro.tex <==
% \section{Introduction}

% Multimodal Large Language Models (MLLMs) have achieved remarkable success in diverse vision-language tasks~\cite{achiam2023gpt, team2023gemini,bai2025qwen2}. However, mastering complex, multi-step reasoning remains a formidable frontier. Geometric reasoning serves as a quintessential testbed for this challenge, as it demands the intricate interplay of visual perception, symbolic abstraction, and rigorous logical deduction~\cite{trinh2024solving, he2024olympiadbench}. While recent specialized solvers like AlphaGeometry and Newclid~\cite{trinh2024solving, sicca2024newclid} have demonstrated human-olympiad level performance, general-purpose MLLMs still struggle to maintain coherent inferential chains, often succumbing to hallucinations or logical gaps. A fundamental impediment to progress in this domain is the limitation of existing evaluation and training paradigms, which rely predominantly on \textit{outcome-based feedback}.

% Current benchmarks for geometric problem-solving, such as GeoQA and Geometry3k~\cite{chen2021geoqa, lu2021inter}, typically treat the reasoning process as a black box. They evaluate models solely on the correctness of the final numerical answer. This outcome-based approach is a coarse proxy for reasoning capability. It suffers from two critical failures: \textit{false positives}, where a model arrives at the correct answer through flawed logic (a "lucky guess"), and \textit{false negatives}, where a sound reasoning process is penalized for a minor calculation error. More importantly, sparse outcome signals fail to provide the granular feedback necessary for models to learn \textit{how} to reason. Recent work in text-based mathematics has shown the efficacy of \textit{process-level verification}~\cite{lightman2023let}, yet applying this to multimodal geometry is hindered by the scarcity of high-quality, step-wise annotated data.

% To bridge this gap, we shift the paradigm from outcome-based assessment to \textit{process-level evaluation and reinforcement}. Our core contribution is a novel framework for geometric reasoning founded on the principle of \textit{step-wise verifiability}. We leverage a formal methods engine, TrustGeoGen~\cite{trustgeogen2025}, to automatically synthesize a benchmark where each problem instance is paired with a complete, formally verified proof skeleton. Unlike standard synthetic data, every intermediate logical step in our skeleton is guaranteed to be correct and sound. We introduce a "proofing-to-solving" transformation that converts abstract logical predicates (e.g., segment congruence) into concrete, automatically verifiable numeric sub-goals.

% This dense, step-level ground truth unlocks a powerful training paradigm aligned with \textit{Reinforcement Learning with Verifiable Rewards (RLVR)}~\cite{deepseek2025deepseek}. We instantiate this via \textit{Process-Aware Verifiable Reward (PAVR)}. Instead of relying on sparse final-answer rewards, we introduce the \textit{Skeleton Rate}—the proportion of correctly achieved intermediate sub-goals—as a dense reward signal. As illustrated in Figure~\ref{fig:pipeline}, this allows us to directly optimize the model's reasoning policy using GRPO~\cite{deepseek2025deepseek}, guiding it towards logically sound and coherent reasoning chains. This approach aligns with the emerging trend of leveraging verifiable computation to enhance reasoning~\cite{deepseek2025deepseek}, extending it for the first time to the multimodal geometric domain.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.0\textwidth]{figures/framework.pdf}
%     \captionof{figure}{\textbf{Framework for benchmark construction and RL training.}
%     \textbf{Data Engine:} TrustGeoGen synthesizes fully verified formal problem instances.
%     \textbf{Decomposition \& Mapping:} The formal skeleton is decomposed into atomic steps, where each predicate is mapped to a numeric target (e.g., congruence $\rightarrow$ length ratio $=1$).
%     \textbf{Reorganization:} These sub-goals are reorganized into a sequential format to provide dense, step-level ground truth.
%     \textbf{PAVR Training:} The model generates structured reasoning chains where each sub-goal is verified. These verification results are converted into dense, process-level rewards to optimize the policy via GRPO.}
%     \label{fig:pipeline}
% \end{figure*}

% Our contributions are threefold:
% \begin{enumerate}
%     \item We construct a new benchmark for multimodal geometric reasoning where every intermediate step is formally verified and automatically checkable, enabling robust, process-level evaluation.
%     \item We propose a novel \textit{Process-Aware Verifiable Reward (PAVR)} framework that leverages verifiable sub-goals to provide dense, process-aware reward signals, significantly improving reasoning consistency.
%     \item We demonstrate through extensive experiments that our method outperforms baselines across geometry, general mathematics, and reasoning benchmarks.
% \end{enumerate}
\section{Introduction}

Multimodal Large Language Models (MLLMs) have achieved remarkable success in diverse vision-language tasks~\cite{achiam2023gpt, team2023gemini,bai2025qwen2}.
However, mastering complex, multi-step reasoning remains a formidable frontier.
Geometric reasoning serves as a quintessential testbed for this challenge, as it demands the intricate interplay of visual perception, symbolic abstraction, and rigorous logical deduction~\cite{trinh2024solving, he2024olympiadbench}.
While recent specialized solvers such as AlphaGeometry and Newclid~\cite{trinh2024solving, sicca2024newclid} have demonstrated human-olympiad level performance, general-purpose MLLMs still struggle to maintain coherent inferential chains, often succumbing to hallucinations or hidden logical gaps.
A fundamental impediment is the limitation of existing evaluation and training paradigms, which rely predominantly on \textit{outcome-based feedback}.

Standard benchmarks for geometric problem solving, such as GeoQA and Geometry3K~\cite{chen2021geoqa, lu2021inter}, typically treat the reasoning process as a black box and evaluate models solely on the correctness of the final numerical answer.
This outcome-based view is a coarse proxy for reasoning capability.
It suffers from two critical failures:
\textit{false positives}, where a model arrives at the correct answer through flawed logic (a ``lucky guess''), and \textit{false negatives}, where a sound reasoning process is penalized for a minor calculation error.
Moreover, sparse final-answer signals provide little guidance on \emph{how} to reason, making it difficult for models to learn robust intermediate steps.
Recent work in text-based mathematics has shown the promise of \textit{process-level verification}~\cite{lightman2023let}, yet extending this paradigm to multimodal geometry has been hampered by the scarcity of trustworthy, step-wise annotated data.

Acquiring such data is challenging for at least three reasons.
First, collecting large-scale geometric proofs with reliable step-level supervision requires strong formal guarantees of correctness.
Second, many geometric arguments admit multiple valid step orders; evaluation should therefore be invariant to benign re-orderings rather than tied to a single canonical script.
Third, intermediate textual explanations are difficult to check automatically, which makes it hard to convert them into stable and trustworthy reward signals.
These obstacles have limited the adoption of process-level rewards in multimodal reasoning—not because they are undesirable, but because they have been practically difficult to obtain.

To address these challenges, we shift the paradigm from outcome-based assessment to \textit{process-level evaluation and reinforcement}.
Our core idea is to ground geometric reasoning in \textit{step-wise verifiability}.
We leverage the formal methods engine TrustGeoGen~\cite{trustgeogen2025} to automatically synthesize a benchmark in which each problem instance is paired with a complete, formally verified proof skeleton.
Unlike standard synthetic data, every intermediate predicate in this skeleton is mechanically checked for logical soundness.
We then apply a ``proofing-to-solving'' transformation that maps abstract predicates (e.g., segment congruence) into concrete, automatically verifiable numeric sub-goals, yielding dense, step-level ground truth for both evaluation and training (Section~\ref{sec:benchmark}).



\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/framework.pdf}
    \captionof{figure}{\textbf{Overall framework for step-wise verifiable geometric reasoning and process-aware training.}
    (\textbf{Top}) \textit{Step-wise verifiable benchmark}: (1) TrustGeoGen~\cite{trustgeogen2025} generates formally verified solution skeletons; (2) each predicate is decomposed and mapped to a numeric sub-goal; (3) sub-goals are reorganized into a sequence that exposes process-aware metrics such as SR and SC, alongside the final goal.
    (\textbf{Bottom}) \textit{PAVR training}: given a problem and its sub-goals, the vision-language model produces structured reasoning traces; each predicted sub-goal is verified against ground truth, and the resulting signals are aggregated into dense process-aware rewards used to optimize the policy via GRPO.}
    \label{fig:pipeline}
\end{figure*}

This representation enables a training paradigm aligned with \textit{Reinforcement Learning with Verifiable Rewards (RLVR)}~\cite{deepseek2025deepseek}.
We instantiate it via a \textit{Process-Aware Verifiable Reward (PAVR)} framework.
Instead of relying on sparse final-answer rewards, we introduce the \textit{Skeleton Rate}---the proportion of correctly achieved sub-goals---as a dense reward signal for geometric reasoning.
As illustrated in Figure~\ref{fig:pipeline}, our system decomposes formal proofs, maps them to numeric targets, and verifies each generated sub-goal to produce verifiable rewards that are optimized with GRPO~\cite{deepseek2025deepseek}.
This approach follows the emerging trend of leveraging verifiable computation to enhance reasoning and extends it, for the first time, to multimodal geometry.
Furthermore, our benchmark supports both process-level metrics---Skeleton Rate (SR) and Skeleton Completion (SC)---and the standard outcome metric of Final Answer (FA).
When used together, these metrics reveal that process-level correctness and final-answer accuracy are only moderately aligned, indicating that outcome-only evaluation can overestimate true reasoning reliability (see Section~\ref{sec:benchmark_eval} for a detailed analysis).



Our contributions are threefold:
\begin{enumerate}
    \item We construct a new benchmark for multimodal geometric reasoning where every intermediate step is formally verified and automatically checkable, enabling robust process-level evaluation with SR and SC, together with standard outcome-based assessment via FA (Section~\ref{sec:benchmark}).
    \item We propose a \textit{Process-Aware Verifiable Reward (PAVR)} framework that leverages verifiable sub-goals to provide dense, process-aware reward signals, and we train MLLMs with GRPO and PPO on this benchmark (Section~\ref{sec:ablation}).
    \item We conduct extensive experiments showing that PAVR-based training improves both final-answer accuracy and independent process-quality metrics across geometry, general mathematics, and broader reasoning benchmarks, consistently outperforming baselines. 
\end{enumerate}


==> sections/04_methods.tex <==
\section{Methodology}
\label{sec:method}

\subsection{Overview}

We convert geometry problems into verifiable multi-step reasoning chains and train models with process-level supervision. During data construction, we leverage formal solution specifications validated by TrustGeoGen~\citep{trustgeogen2025} to derive a sequence of numeric sub-goals aligned with proof steps. At training and inference time, models observe the problem (image + text) and output structured answers for all sub-goals; these answers are checked against verified targets to compute skeleton-based metrics (Section~\ref{sec:eval_metrics}) and process rewards for reinforcement learning (Section~\ref{sec:rlvr}).

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{/figure}
%   \caption{End-to-end pipeline. Left: data generation and conversion—formal skeleton validation with TrustGeoGen and predicate-to-numeric mapping to obtain verifiable sub-goals. Right: training/inference from problem statements; per-step correctness is aggregated into skeleton-based metrics and process rewards.}
%   \label{fig:pipeline}
% \end{figure}

\subsection{Task Definition}

\paragraph{Input and output}
Given a multimodal geometry problem (image + text), the model produces a structured response:
\begin{itemize}
  \item A \texttt{<think>} block containing reasoning steps and explanations.
  \item An \texttt{<answer>} block listing numeric values for all sub-goals $[T_0, T_1, \ldots, T_{N-1}]$.
\end{itemize}
Each sub-goal $T_i$ is explicitly stated in the prompt as a numeric target (e.g., ``$T_0 = |AC|/|BC|$'', ``$T_1 = \angle(AB,AC) - \angle(BC,AB)$ in degrees mod 180'').

\paragraph{Evaluation and training}
For evaluation, we compare the model's numeric answers $\{\hat{y}_i\}$ against verified ground truth $\{y_i\}$ using robust numeric equivalence (Section~\ref{sec:skeleton_scoring}). For training, we use these per-step correctness signals as process rewards (Section~\ref{sec:rlvr}).

\subsection{Data Generation and Conversion Pipeline}
\label{sec:pipeline}

We use formal solution specifications during data construction to obtain verified ground truth and to ensure that sub-goal targets are aligned with proof steps. The pipeline consists of three stages:

\paragraph{(1) Formal skeleton validation}
We parse the formal solution specification into an ordered list of inference steps $\{\mathcal{S}_t\}_{t=1}^{T}$, each stating a geometric predicate (e.g., segment congruence, equal angles, parallelism) over arguments (points, segments, angles). TrustGeoGen~\citep{trustgeogen2025} validates step-level correctness (predicate support, argument types/arity) and enforces cross-step consistency.

\paragraph{(2) Geometric-to-numeric mapping}

Each geometric predicate is mapped to one or more numeric targets with expected values; angles are evaluated modulo $180^{\circ}$ and ratios are dimensionless. Representative examples:

\begin{itemize}
  \item Segment congruence: $T=\frac{|AB|}{|CD|} \Rightarrow 1$.
  \item Equal angles: $T=\angle(AB,CD)-\angle(EF,GH) \Rightarrow 0$ (mod 180°).
  \item Parallel lines: $T=\angle(AB,CD) \Rightarrow 0$ (mod 180°).
  \item Collinearity: $T=\mathrm{area\_triangle}(A,B,C) \Rightarrow 0$.
\end{itemize}

The complete mapping table and corner cases (e.g., orientation, degenerate configurations) appear in Appendix~\ref{app:mapping}.

\paragraph{(3) Prompt generation}
For each instance, we generate a prompt that (i) describes the problem setup (image + text), (ii) explicitly lists all sub-goals $T_0, T_1, \ldots$ derived from the formal steps, and (iii) requests a structured response with reasoning and numeric answers. We retain the prompt paired with verified numeric targets $\{y_i\}$.

\paragraph{Quality control}
We apply numeric-equivalence checks (angles modulo $180^{\circ}$; tolerance $\epsilon=0.02$) and cross-step consistency checks to ensure the derived targets are verifiable, mutually consistent, and faithful to the skeleton.

\subsection{Skeleton-Based Scoring}
\label{sec:skeleton_scoring}

Let $\hat{y}_i$ be the model's output for sub-goal $i$ and $y_i$ the ground truth. We use a robust equivalence test $\mathrm{eq}(\cdot)$ that
(i) accepts algebraic/numeric equivalence (e.g., $1/2=0.5$, $\sqrt{2}\!\approx\!1.414$),
(ii) evaluates angles modulo $180^{\circ}$,
(iii) permits decimal approximations within tolerance $\epsilon=0.02$.

For a reasoning chain with $N$ sub-goals, the skeleton rate is computed as:
\[
s_{\text{rate}}(y)=\frac{1}{N}\sum_{i=1}^{N}\mathbb{I}\!\big(\mathrm{eq}(\hat{y}_i,y_i)\big)\in[0,1],
\]
representing the proportion of correctly answered sub-goals. This fine-grained metric serves as both our primary evaluation metric (Section~\ref{sec:eval_metrics}) and the foundation for process-level reward signals in reinforcement learning (Section~\ref{sec:rlvr}).

\subsection{Reinforcement Learning with Verifiable Process Rewards}
\label{sec:rlvr}

We formulate multi-step geometric reasoning as a contextual bandit problem where the agent (policy $\pi_\theta$) generates a complete structured response given a problem statement, and receives scalar feedback based on the correctness of intermediate reasoning steps. Unlike outcome-based RL methods that only reward final-answer correctness, our approach provides fine-grained process-level rewards through verified sub-goal evaluation.

\paragraph{Problem formulation}
Given a problem $x$, the policy $\pi_\theta$ generates a structured response $y$ containing reasoning steps and numeric answers for all sub-goals. We model this as a single-episode Markov Decision Process with:
\begin{itemize}
  \item \textbf{State space}: Problem statement $x$ (image + text + sub-goal specifications).
  \item \textbf{Action space}: Structured response $y$ (\texttt{<think>} block + \texttt{<answer>} block).
  \item \textbf{Reward function}: Skeleton rate $r(x,y) = s_{\text{rate}}(y)$, computed by verifying each sub-goal answer against ground truth.
\end{itemize}
This single-step formulation ($\gamma=1$, $\lambda=1$) is appropriate because the entire reasoning chain is generated autoregressively before receiving any feedback, and the reward comprehensively evaluates the full reasoning process.

\paragraph{Policy optimization with PPO}
We optimize the policy using Proximal Policy Optimization~\citep{schulman2017proximal}, chosen for its stability and effectiveness in language model fine-tuning. Starting from a pretrained checkpoint $\pi_{\mathrm{ref}}$, we iteratively collect rollouts and update the policy $\pi_\theta$ to maximize expected rewards while constraining deviation from the reference policy.

For each problem $x$, we sample $K$ responses $\{y_k\}_{k=1}^{K}$ from the current policy and compute their skeleton rates $\{r_k\}_{k=1}^{K}$. The PPO objective combines clipped policy gradient updates with a KL penalty:
\[
\mathcal{L}_{\mathrm{PPO}}(\theta)=\mathbb{E}_{x,k}\Big[\min\!\big(\rho_k A_k,\;\mathrm{clip}(\rho_k,1-\epsilon_{\text{clip}},1+\epsilon_{\text{clip}})A_k\big)\Big]
\;-\;\beta\,\mathrm{KL}\!\big(\pi_\theta(\cdot|x)\,\|\,\pi_{\mathrm{ref}}(\cdot|x)\big),
\]
where $\rho_k = \exp\!\big(\log\pi_\theta(y_k|x)-\log\pi_{\theta_{\mathrm{old}}}(y_k|x)\big)$ is the importance sampling ratio, $A_k$ is the advantage estimate (detailed below), $\epsilon_{\text{clip}}=0.2$ is the clipping threshold, and $\beta=10^{-2}$ controls the strength of the KL penalty.

\paragraph{Group-normalized advantage estimation}
A key challenge in using skeleton rate as a reward signal is its high variance: different problems exhibit vastly different baseline difficulty, leading to incomparable absolute reward scales. To address this, we employ \textit{group normalization}—computing advantages within the $K$ samples of each problem instance rather than across the entire batch.

For each problem $x$ with samples $\{r_k\}_{k=1}^{K}$, we compute group statistics:
\[
\mu_x=\frac{1}{K}\sum_{k=1}^{K}r_k,\quad
\sigma_x=\sqrt{\frac{1}{K}\sum_{k=1}^{K}(r_k-\mu_x)^2},
\]
and normalize advantages:
\[
A_k=\frac{r_k-\mu_x}{\sigma_x+\epsilon},
\]
where $\epsilon=10^{-8}$ prevents division by zero. This normalization ensures that (1) the policy learns to prefer better reasoning strategies \textit{within} each problem context, and (2) training gradients remain stable across problems of varying difficulty.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{/figure}
  \caption{Reinforcement learning with verifiable process rewards. For each problem, $K$ structured responses are sampled and evaluated by the verifier; skeleton rates are group-normalized into advantages and optimized with clipped PPO plus a reference-KL penalty.}
  \label{fig:rlvr}
\end{figure}

==> sections/08_dataset.tex <==
\section{Dataset and Benchmark}

\label{sec:benchmark}

\subsection{Motivation and Key Features}

Existing geometry benchmarks primarily focus on final-answer evaluation, lacking the infrastructure to assess intermediate reasoning steps or provide process-level training signals. 
This limitation hinders the development of models that genuinely learn multi-step reasoning rather than pattern matching to final answers.

We introduce a benchmark with three distinguishing features:

\noindent\textbf{(1) Formal verification}: Each problem includes a formally validated solution skeleton verified by TrustGeoGen~\citep{fu2025trustgeogen}, ensuring that every reasoning step is logically sound and consistent. This enables reliable ground truth for intermediate steps, not just final answers.
\noindent\textbf{(1) Formal verification}: Each problem includes a formally validated solution skeleton verified by TrustGeoGen~\citep{fu2025trustgeogen}, ensuring that every reasoning step is logically sound and consistent. This enables reliable ground truth for intermediate steps, not just final answers.

\noindent\textbf{(2) Verifiable sub-goal decomposition}: We map geometric predicates to numeric targets with verified ground truth, allowing automatic evaluation of each reasoning step without human annotation. This transformation makes process-level evaluation practical at scale.

\noindent\textbf{(3) Process-level metrics}: We introduce skeleton-based evaluation metrics (Section~\ref{sec:eval_metrics}) that quantify reasoning quality at the granularity of individual sub-goals, enabling both fine-grained assessment and process-reward training signals for reinforcement learning.

Together, these features enable systematic investigation of multi-step reasoning capabilities and process-level supervision—capabilities absent in existing geometry benchmarks that focus solely on outcome evaluation.

\subsection{Construction Pipeline and Dataset Characteristics}

Our training set and test benchmark are constructed following the pipeline detailed in Section~\ref{sec:pipeline}: (i) formal skeleton validation with TrustGeoGen, (ii) geometric-to-numeric mapping, and (iii) quality control with numeric-equivalence checks.
The key innovation is the transformation of geometric predicates into verifiable numeric targets, enabling automatic verification of intermediate reasoning steps—a critical enabler for both process-level evaluation and reinforcement learning with dense supervision signals.

We release balanced splits: Train = 221 instances, Test = 256 instances.
Despite the modest size, the formal verification and sub-goal decomposition provide rich supervision: each instance contains multiple verifiable reasoning steps, yielding dense training signals for process-level learning.

\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.95\textwidth]{figures/problem_fl_distribution_comparison.pdf}
  \vspace{1mm}
  
  \includegraphics[width=0.95\textwidth]{figures/proof_length_comparison.pdf}
  \vspace{-2mm}
  \caption{\textbf{Dataset characteristics.} \textbf{Top}: Problem element distribution shows comparable coverage of geometric constructions (parallelograms, triangles, circles, etc.) across Train and Test splits, ensuring consistent concept representation. \textbf{Bottom}: Proof-length distribution reveals that the test set is skewed toward longer reasoning chains (mean length: Train = 3.8, Test = 4.2), providing a more challenging evaluation while maintaining distributional overlap with training data. This design enables assessment of generalization to harder multi-step problems.}
  \label{fig:dataset_dists}
\end{figure*}

Figure~\ref{fig:dataset_dists} illustrates key distributional properties of our benchmark.
The element distribution (top) demonstrates matched coverage of fundamental geometric constructions across both splits, with top-10 element types exhibiting similar proportions. This ensures models are evaluated on concepts represented during training.
The proof-length distribution (bottom) shows that while both splits share overlapping ranges, the test set emphasizes longer reasoning chains, creating a difficulty gradient that tests generalization beyond memorized patterns.

\subsection{Evaluation Metrics}

\label{sec:eval_metrics}

A key contribution of our work is the introduction of fine-grained, process-level evaluation for multi-step geometric reasoning. 
We propose two skeleton-based metrics—\textbf{Skeleton Rate} and \textbf{Skeleton Completion}—which assess reasoning quality at the granularity of individual sub-goals rather than only final outcomes.
We additionally report \textbf{Final Answer}, a standard outcome-based metric, to provide comprehensive evaluation.
All metrics are reported as percentages.

\paragraph{Skeleton Rate}
Multi-step geometric reasoning requires models to correctly answer a sequence of sub-goals that form the reasoning skeleton.
Skeleton Rate measures the proportion of correctly answered sub-goals across the entire reasoning process.

Formally, for a proof chain containing $n_i$ sub-goals in instance $i$, Skeleton Rate is defined as:
\[
\text{Skeleton Rate} = \frac{1}{N} \sum_{i=1}^{N} \frac{\text{\# correct sub-goals in instance } i}{n_i}
\]
where $N$ is the total number of test instances.
This fine-grained metric evaluates each intermediate sub-goal, providing process-level insight into reasoning quality.

\paragraph{Skeleton Completion}
Skeleton Completion measures whether a model correctly answers \textit{all} sub-goals in a proof chain:
\[
\text{Skeleton Completion} = \frac{1}{N} \sum_{i=1}^{N} \mathbb{1}[\text{all } n_i \text{ sub-goals in instance } i \text{ are correct}]
\]
This strict, binary metric reflects end-to-end reasoning consistency.
Due to its all-or-nothing nature, Skeleton Completion scores are typically substantially lower than Skeleton Rate.

\paragraph{Final Answer}
Final Answer measures task-level success by evaluating only the last sub-goal:
\[
\text{Final Answer} = \frac{1}{N} \sum_{i=1}^{N} \mathbb{1}[\text{last sub-goal in instance } i \text{ is correct}]
\]
This outcome-based metric represents standard task accuracy but does not capture the quality of intermediate reasoning steps.

==> tables/ablation-reward-old.tex <==
\begin{table*}[t]
\centering
\small
\caption{Ablation study of reward formulations (Final Answer, Skeleton Completion, Skeleton Rate) on Qwen2.5-VL-7B-Instruct and Qwen2.5-VL-3B-Instruct across benchmarks. For each model size, Skeleton Rate achieves the best overall average and is consistently competitive across domains, while Skeleton Completion can be favorable on some benchmarks. Best results within each model size are in \textbf{bold}, second-best are \underline{underlined}. $\Delta$ denotes the improvement of Skeleton Rate over Final Answer.}
\label{tab:ablation}
\begin{adjustbox}{width=0.92\linewidth}
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{\textbf{Benchmark}} & \multicolumn{4}{c}{\textbf{Qwen2.5-VL-7B} trained on} & \multicolumn{4}{c}{\textbf{Qwen2.5-VL-3B} trained on} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& \textbf{FA Reward} & \textbf{SC Reward} & \textbf{SR Reward} & \textbf{$\Delta$} & \textbf{FA Reward} & \textbf{SC Reward} & \textbf{SR Reward} & \textbf{$\Delta$} \\
\midrule
\multicolumn{9}{l}{\textbf{\textit{Geometry Reasoning}}} \\
\midrule
GeoGoal (SC) & 5.9 & \underline{9.4} & \textbf{15.2} & \cellcolor{green!15}+9.3 & 5.9 & \underline{9.4} & \textbf{13.7} & \cellcolor{green!15}+7.8 \\
GeoGoal (SR) & \underline{79.1} & 82.1 & \textbf{87.7} & \cellcolor{green!15}+8.6 & \underline{79.1} & 67.5 & \textbf{83.1} & \cellcolor{green!15}+4.0 \\
GeoGoal (CR) & \underline{7.4} & 11.4 & \textbf{17.4} & \cellcolor{green!15}+10.0 & \underline{7.4} & 13.9 & \textbf{16.4} & \cellcolor{green!15}+9.0 \\
GeoQA & \underline{54.4} & 53.9 & \textbf{58.2} & \cellcolor{green!15}+3.8 & 48.0 & \underline{48.3} & \textbf{50.1} & \cellcolor{green!15}+2.1 \\
Geometry3K & 36.7 & \underline{36.8} & \textbf{40.3} & \cellcolor{green!15}+3.6 & \underline{27.0} & 26.0 & \textbf{29.8} & \cellcolor{green!15}+2.8 \\
GeoPQA-Test & \underline{77.9} & 77.5 & \textbf{82.1} & \cellcolor{green!15}+4.2 & 72.2 & \underline{74.2} & \textbf{75.6} & \cellcolor{green!15}+3.4 \\
GeoPQA-Valid & \underline{42.6} & 40.8 & \textbf{59.4} & \cellcolor{green!15}+16.8 & \underline{57.6} & 57.4 & \textbf{57.8} & \cellcolor{green!15}+0.2 \\
TrustGeo-Test & \underline{20.8} & 19.6 & \textbf{25.4} & \cellcolor{green!15}+4.6 & \underline{20.0} & 13.8 & \textbf{20.8} & \cellcolor{green!15}+0.8 \\
OlympiadBench & \underline{27.7} & 24.1 & \textbf{32.1} & \cellcolor{green!15}+4.4 & \underline{21.4} & 21.4 & \textbf{24.1} & \cellcolor{green!15}+2.7 \\
% \cdashline{1-9}
\textit{Geometry Average} & \underline{40.2} & 38.9 & \textbf{50.7} & \cellcolor{green!15}+10.5 & \underline{38.2} & 37.7 & \textbf{44.5} & \cellcolor{green!15}+6.3 \\
\midrule
\multicolumn{9}{l}{\textbf{\textit{General Mathematics}}} \\
\midrule
AMC & 31.3 & \underline{33.7} & \textbf{38.6} & \cellcolor{green!15}+7.3 & \underline{31.3} & 28.9 & \textbf{34.9} & \cellcolor{green!15}+3.6 \\
MATH 500 & 61.2 & \textbf{65.6} & \underline{63.2} & \cellcolor{green!15}+2.0 & \underline{56.6} & 54.6 & \textbf{59.0} & \cellcolor{green!15}+2.4 \\
% \cdashline{1-9}
\textit{General Math Average} & 46.3 & \underline{49.7} & \textbf{50.9} & \cellcolor{green!15}+4.6 & \underline{44.0} & 41.8 & \textbf{47.0} & \cellcolor{green!15}+3.0 \\
\midrule
\multicolumn{9}{l}{\textbf{\textit{General Reasoning}}} \\
\midrule
LiveBench-Reasoning & 17.5 & \textbf{25.0} & \underline{20.0} & \cellcolor{green!15}+2.5 & \underline{17.5} & 13.5 & \textbf{19.5} & \cellcolor{green!15}+2.0 \\
VisuLogic & 25.6 & \underline{26.5} & \textbf{28.5} & \cellcolor{green!15}+2.9 & \underline{25.1} & 25.0 & \textbf{27.3} & \cellcolor{green!15}+2.2 \\
% \cdashline{1-9}
\textit{General Reasoning Average} & 21.6 & \textbf{25.8} & \underline{24.3} & \cellcolor{green!15}+2.7 & \underline{21.3} & 19.3 & \textbf{23.4} & \cellcolor{green!15}+2.1 \\
\midrule
\textbf{Overall Average} & 35.7 & \underline{38.1} & \textbf{41.5} & \textbf{\cellcolor{green!15}+5.8} & \underline{32.3} & 31.4 & \textbf{38.6} & \textbf{\cellcolor{green!15}+6.3} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}
